Anomalous production of massive gauge boson pairs at muon colliders

The prospects of searches for anomalous production of hadronically decaying weak boson pairs at proposed high-energy muon colliders are reported. Muon-muon collision events are simulated at $\sqrt{s}=6$, 10, and 30 TeV, corresponding to an integrated luminosity of $4$, $10$, and $10$ ab$^{-1}$, respectively. Simulated $\mu\mu\rightarrow\mathrm{W}\mathrm{W}+\nu\nu/\mu\mu$ events are used to set expected constraints on the structure of quartic vector boson interactions in the framework of a dimension-8 effective field theory. Similarly, $\mu\mu\rightarrow\mathrm{W}\mathrm{W}/\mathrm{Z}\mathrm{Z}+\nu\nu$ events are used to report constraints on the product of the cross section and branching fraction for vector boson fusion production of a heavy neutral Higgs boson decaying to weak boson pairs. These results are interpreted in the context of the Georgi-Machacek model.

==> Sections/results.tex <==
\section{Results}
\label{S:results}

The selected events are used to constrain aQGC parameters in an EFT framework. Statistical analysis of the event yields is performed separately in the $\PW\PW\nu\nu$ and $\PW\PW\mu\mu$ channels with a fit to the invariant mass distribution of the two leading jets, which typically correspond to the pair of $\PW$ bosons, denoted $m_{\PW\PW}$. The distributions of $m_{\PW\PW}$ after the event selection at each of the different center-of-mass energies are shown in Fig.~\ref{fig:dijet_mass}. The expected $95\%$ confidence level (CL) lower and upper limits on the aQGC parameters $f/\Lambda^4$, where $f$ is the Wilson coefficient of the given operator and $\Lambda$ is the energy scale of new physics, are derived from Wilk's theorem~\cite{wilks:10.1214} assuming that the profile likelihood test statistic is $\chi^2$ distributed~\cite{CLs}. No nuisance parameters corresponding to systematic uncertainties are included in the fits. 

\begin{figure}[htbp]
\centering
\includegraphics[width=0.38\textwidth]{Figures/nunu_6TeV.pdf} 
\includegraphics[width=0.38\textwidth]{Figures/mumu_6TeV.pdf}
\includegraphics[width=0.38\textwidth]{Figures/nunu_10TeV.pdf} 
\includegraphics[width=0.38\textwidth]{Figures/mumu_10TeV.pdf}
\includegraphics[width=0.38\textwidth]{Figures/nunu_30TeV.pdf} 
\includegraphics[width=0.38\textwidth]{Figures/mumu_30TeV.pdf}
\caption{Distributions of $m_{\PW\PW}$ after the event selection in the $\PW\PW\nu\nu$ (left) and $\PW\PW\mu\mu$ (right) channels for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV (upper), 10 TeV (middle), and 30 TeV (lower). The filled histograms show the background expectation, while the solid lines show the separate contributions from the interference (red) and quadratic (green) terms for a  value of the \texttt{T1} parameter at the limit of the expected sensitivity. %The overflow is included in the last bin.
}
\label{fig:dijet_mass}
\end{figure}

Table~\ref{tab:limits_nunu} shows the individual lower and upper limits obtained by setting all other aQGC parameters to zero in the $\PW\PW\nu\nu$ channel for the \texttt{S0}, \texttt{S1}, \texttt{M0}, \texttt{M1}, \texttt{M7}, \texttt{T0}, \texttt{T1}, and \texttt{T2} operators, at each of the different center-of-mass energies. The $\PW\PW\mu\mu$ contribution in the $\PW\PW\nu\nu$ channel is treated as a background process and assumed to be purely SM in the statistical analysis. Table~\ref{tab:limits_mumu} shows the individual lower and upper limits obtained by setting all other aQGC parameters to zero in the $\PW\PW\mu\mu$ channel for the \texttt{T0}, \texttt{T1}, \texttt{T2}, \texttt{T6}, and \texttt{T7} operators for the different center-of-mass energies. The operators \texttt{T6} and \texttt{T7} are especially interesting for the $\PW\PW\mu\mu$ channel as the presence of these operators does not modify the SM quartic $\PW\PW\PW\PW$ vertex. 


\begin{table}[htb]
\centering
\caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators \texttt{S0}, \texttt{S1}, \texttt{S2}, \texttt{M0}, \texttt{M1}, \texttt{M7}, \texttt{T0}, \texttt{T1}, and \texttt{T2} in the $\PW\PW\nu\nu$ channel for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV, 10 TeV, and 30 TeV. The energy at which tree-level unitarity would be violated for these parameter values is also shown.}\label{tab:limits_nunu}
\vspace{0.3cm}
\scriptsize
\begin{tabular}{c|cc|cc|cc}
\toprule
$\PW\PW\nu\nu$ &\multicolumn{2}{c|}{6~TeV}&\multicolumn{2}{c|}{10~TeV} &\multicolumn{2}{c}{30~TeV}\\
 & Limit & Unitarity & Limit & Unitarity & Limit & Unitarity \\
 &  (TeV\(^{-4}\)) & Bound (TeV)  &  (TeV\(^{-4}\)) & Bound (TeV)  &  (TeV\(^{-4}\)) & Bound (TeV) \\
\midrule
 %\(f_{\mathrm{M},0}/\Lambda^4\) & \([-0.025, 0.027]\) & \([5.9, 5.8]\)  \\
 %\(f_{\mathrm{M},1}/\Lambda^4\) &  \([-0.063, 0.052]\) & \([6.6, 6.9]\) \\
 %\(f_{\mathrm{M},7}/\Lambda^4\) &  \([-0.094, 0.12]\) & \([7.1, 6.7]\) \\
 %\(f_{\mathrm{S},0}/\Lambda^4\) &  \([-0.19, 0.18]\) & \([3.8, 4.4]\) \\
 %\(f_{\mathrm{S},1}/\Lambda^4\) &  \([-0.11, 0.11]\) & \([4.5, 4.3]\) \\
 %\(f_{\mathrm{S},2}/\Lambda^4\) &  \([-0.11, 0.11]\) & \([4.4, 4.3]\) \\
 %\(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.0049, 0.0025]\) & \([6.2, 6.3]\) \\
 %\(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.0017, 0.0014]\) & \([7.7, 8.1]\) \\
 %\(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.0011, 0.0046]\) & \([6.6, 7.0]\) \\
  \(f_{\mathrm{M},0}/\Lambda^4\) & \([-0.025, 0.027]\) & \([5.9, 5.8]\) &    \([-0.0048, 0.0049]\) & \([8.9, 8.8]\)   &        \([-0.00046, 0.00046]\) & \([15.8, 15.8]\)   \\
 \(f_{\mathrm{M},1}/\Lambda^4\) &  \([-0.063, 0.052]\) & \([6.6, 6.9]\) &      \([-0.0096, 0.0084]\) & \([10.5, 10.8]\)  &    \([-0.0012, 0.0011]\) & \([17.6, 17.8]\)     \\ 
 \(f_{\mathrm{M},7}/\Lambda^4\) &  \([-0.094, 0.12]\) & \([7.1, 6.7]\) &       \([-0.016, 0.019]\) & \([10.9, 10.6]\)  &      \([-0.0021, 0.0022]\) & \([18.1, 17.9]\)     \\ 
 \(f_{\mathrm{S},0}/\Lambda^4\) &  \([-0.19, 0.18]\) & \([3.8, 4.4]\) &        \([-0.034, 0.033]\) & \([5.8, 6.8]\)  &        \([-0.0046, 0.0045]\) & \([9.5, 10.9]\)      \\ 
 \(f_{\mathrm{S},1}/\Lambda^4\) &  \([-0.11, 0.11]\) & \([4.5, 4.3]\) &        \([-0.019, 0.019]\) & \([6.8, 6.6]\)  &        \([-0.0025, 0.0025]\) & \([11.3, 10.9]\)     \\ 
 \(f_{\mathrm{S},2}/\Lambda^4\) &  \([-0.11, 0.11]\) & \([4.4, 4.3]\) &        \([-0.019, 0.019]\) & \([6.8,  6.6]\)  &       \([-0.0025, 0.0025]\) & \([11.3, 10.9]\)     \\ 
 \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.0049, 0.0025]\) & \([6.2, 6.3]\) &    \([-0.00070, 0.00051]\) & \([10.0, 9.3]\)  &   \([-0.000072, 0.000062]\) & \([17.7, 15.7]\) \\  
 \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.0017, 0.0014]\) & \([7.7, 8.1]\) &    \([-0.00089, 0.00053]\) & \([9.0, 10.3]\)  &   \([-0.000095, 0.000082]\) & \([15.5, 16.3]\) \\  
 \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.011, 0.0046]\) & \([6.6, 7.0]\) &    \([-0.0015, 0.00082]\) & \([10.8, 10.7]\)  &    \([-0.00017, 0.00013]\) & \([18.4, 16.7]\)   \\ 
\bottomrule
\end{tabular}
\end{table}

%Expected lower and upper 95\% CL limits on the parameters of the quartic operators \texttt{S0}, \texttt{S1}, \texttt{S2}, \texttt{M0}, \texttt{M1}, \texttt{M7}, \texttt{T0}, \texttt{T1}, and \texttt{T2} in the $\PW\PW\nu\nu$ channel for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV, $\sqrt{s}=10$ TeV, and $\sqrt{s}=30$ TeV. The energy at which the tree-level unitarity would be violated for the allowed parameter values is also shown.
\begin{table}[htb]
\centering
\caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators \texttt{T0}, \texttt{T1}, \texttt{T2}, \texttt{T6}, \texttt{T7} in the $\PW\PW\mu\mu$ channel for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV, 10 TeV, and 30 TeV. The energy at which tree-level unitarity would be violated for these parameter values is also shown. \label{tab:limits_mumu}}
\vspace{0.3cm}
\scriptsize
\begin{tabular}{c|cc|cc|cc}
\toprule
$\PW\PW\mu\mu$ &\multicolumn{2}{c|}{6~TeV}&\multicolumn{2}{c|}{10~TeV} &\multicolumn{2}{c}{30~TeV}\\
 & Limit & Unitarity & Limit & Unitarity & Limit & Unitarity \\
 &  (TeV\(^{-4}\)) & Bound (TeV)  &  (TeV\(^{-4}\)) & Bound (TeV)  &  (TeV\(^{-4}\)) & Bound (TeV) \\
\midrule
\(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.0065, 0.0026]\) & \([8.7, 10.9]\)   & \([-0.0012, 0.00057]\) & \([13.2, 15.8]\)     & \([-0.000031, 0.000018]\) & \([32.2, 36.8]\) \\
\(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.036, 0.024]\) & \([4.2, 5.2]\)      & \([-0.0020, 0.00089]\) & \([8.6, 11.9]\)      & \([-0.000050, 0.000031]\) & \([21.1, 27.0]\) \\
\(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.052, 0.030]\) & \([5.2, 6.7]\)      & \([-0.0068, 0.0012]\) & \([8.6, 15.1]\)       & \([-0.000091, 0.000042]\) & \([24.8, 35.1]\) \\
\(f_{\mathrm{T},6}/\Lambda^4\) &  \([-0.0052, 0.0041]\) & \([10.0, 11.1]\)  & \([-0.00090, 0.00074]\) & \([15.5, 16.9]\)    & \([-0.000027, 0.000024]\) & \([37.1, 40.1]\) \\
\(f_{\mathrm{T},7}/\Lambda^4\) &  \([-0.0068, 0.0042]\) & \([12.8, 15.0]\)  & \([-0.0011, 0.00086]\) & \([19.9, 22.3]\)     & \([-0.000034, 0.000028]\) & \([47.8, 52.7]\) \\
\bottomrule
\end{tabular}
\end{table}

The EFT framework is not a complete model and the presence of nonzero aQGCs will violate tree-level unitarity at sufficiently high energy~\cite{Almeida:2020ylr}. The physicality of the obtained limits can be deduced by investigating the perturbative partial-wave unitarity. While detailed studies on the EFT framework validity are beyond the scope of this paper, the unitarity bounds were evaluated for each aQGC parameter limit by calculating the $\PV\PV$ center-of-mass energy at which the tree-level unitarity would be violated without a form factor using \textsc{vbfnlo} 1.4.0~\cite{Arnold:2008rz,Arnold:2011wj,Baglio:2014uba}. These unitarity bounds are shown in Tables~\ref{tab:limits_nunu} and~\ref{tab:limits_mumu}. Various $\PV\PV \to \PV\PV $ channel contributions to the zeroth partial wave are considered and the smallest unitarity bound is chosen.  Generally, for 6 and 10 TeV collider options, unitarity violation occurs around or above the collider center-of-mass energy. 
 %It can be seen that there are no EFT contributions with $m_{\PV\PV}$ values above the unitarity bound for the expected limits for the M1, M7, T0, T1, and T2 (T0, T6, and T7) operators in the $\PW\PW\nu\nu$ ($\PW\PW\mu\mu$) channel at $\sqrt{s}=6$ TeV. 
On the other hand, the expected limits at $\sqrt{s} = 30$~TeV are somewhat optimistic as the corresponding unitarity bounds are significantly smaller than $30$ TeV for many of the operators. 

These results give stringent constraints on the aQGC parameters for the \texttt{S0}, \texttt{S1}, \texttt{M0}, \texttt{M1}, \texttt{M6}, \texttt{M7}, \texttt{T0}, \texttt{T1}, \texttt{T2}, \texttt{T5}, and \texttt{T6} operators. Depending on the operator, the expected limits are better by more than one or two orders of magnitude compared to the expected limits at the HL-LHC and HE-LHC, as reported in Ref.~\cite{Dainese:2703572}, and summarized in Table~\ref{tab:LHC}. The expected limits in the $\PW\PZ$ channel are based on a measurement of fully-leptonic WZ scattering by the ATLAS Collaboration using $\pp$ collisions at $\sqrt{s}=13$~TeV~\cite{Aaboud_2019} with additional cuts to enhance the sensitivity to new physics, while those in the $\PW^{\pm}\PW^{\pm}$ channel are based on simulated $\pp$ collisions with same-sign leptons at $\sqrt{s}=14$~TeV~\cite{ATL-PHYS-PUB-2018-052} with an upgraded ATLAS detector~\cite{ATL-PHYS-PUB-2019-005}. Results for the HE-LHC are obtained based on simulations at $\sqrt{s}=27$~TeV, assuming the same signal-to-background ratio as at the LHC. A few of these LHC results address the unitarity issues in some form, but not all of them. Expected sensitivity to aQGCs at a $\sqrt{s} = 30$~TeV $\mu^{+}\mu^{-}$ collider in the $\PW\PW\nu\nu$ channel using events with leptonically-decaying $\PW$ bosons is reported in Ref.~\cite{Yang:2022fhw}.  Sensitivity to aQGCs at high-energy $e^{+}e^{-}$ colliders are reported in Refs.~\cite{Dainese:2703572,Fleper:2016frz}. 

% The effects of the beam induced backgrounds are also not included.

\begin{table}[htbp]\caption{Summary of expected limits (in TeV$^{-4}$) on the parameters of quartic operators at the HL-LHC and HE-LHC~\cite{Dainese:2703572}.}

\begin{tabular}{|c|c|c|c|c|} \hline
& \multicolumn{2}{|c|}{HL-LHC} & \multicolumn{2}{|c|}{HE-LHC} \\
& $\PW\PZ$ & $\PW^{\pm}\PW^{\pm}$ & $\PW\PZ$ & $\PW^{\pm}\PW^{\pm}$ \\ \hline\hline
$f_{S0}/\Lambda^4$ & [$-8, 8$] & [$-6,6 $] & [$-1.5,1.5 $] & [$-1.5,1.5 $]\\
$f_{S1}/\Lambda^4$ & [$-18,18$] & [$-16,16 $] & [$-3,3 $] & [$-2.5,2.5 $]\\
$f_{T0}/\Lambda^4$ & [$-0.76,0.76$] & [$-0.6,0.6 $] & [$-0.04,0.04 $] & [$-0.027,0.027 $]\\
$f_{T1}/\Lambda^4$ & [$-0.50,0.50$] & [$-0.4,0.4 $] & [$-0.03,0.03 $] & [$-0.016,0.016 $]\\
$f_{M0}/\Lambda^4$ & [$-3.8, 3.8$] & [$-4.0,4.0 $] & [$-0.5,0.5 $] & [$-0.28,0.28 $]\\
$f_{M1}/\Lambda^4$ & [$-5.0,5.0$] & [$-12,12 $] & [$-0.8,0.8 $] & [$-0.90,0.90 $]\\ \hline
\end{tabular}
\label{tab:LHC}
\end{table}

The selected events are also used to derive constraints on resonant neutral Higgs boson production in the GM model.  Statistical analysis of the event yields is again performed with a fit to the invariant mass distribution of the leading dijets, which typically correspond to the pair of $\PV$ bosons, denoted $m_{\PV\PV}$. The distributions of $m_{\PV\PV}$ after the event selection are shown in Fig.~\ref{fig:dijet_mass_higgs}. Exclusion intervals are derived using the CLs method~\cite{Junk:1999kv,Read1} in the asymptotic method for the test statistic~\cite{Cowan:2010js}. The exclusion limits on the product of the cross section of neutral Higgs boson production in association with neutrinos and branching fraction to $\PV\PV$, $\sigma (\PH_{5}\nu\nu) \mathcal{B}(\PH_{5} \to \PV\PV)$, at 95\% CL as a function of $m_{\PH_{5}}$ are shown in Fig.~\ref{fig:gm_limits} (left).  %The results are also interpreted in the context of the GM model. 
The excluded $s_{\PH_5}$ values at 95\% CL in the GM model as a function of $m_{\PH_{5}}$ are shown in Fig.~\ref{fig:gm_limits} (right). The feature seen in the limit plots at $m_{\PH_5}=0.9$~TeV is the transition point between the $s_{\PH}$ values in the \texttt{H5plane} benchmark~\cite{LHCHiggsCrossSectionWorkingGroup:2016ypw}  and is a consequence of the non-negligible effect of the $\PH_5$ width in the statistical analysis. The reported expected $s_{\PH}$ exclusion values are significantly more stringent compared to the exclusion limits of the current LHC results with more than order an of magnitude better sensitivity for $m_{\PH_{5}}$ values greater than 1 TeV~\cite{PhysRevLett.114.231801,Sirunyan:2017sbn,Sirunyan:2017ret,Sirunyan:2019ksz,Sirunyan:2019der,CMS:2021wlt,ATLAS:2022zuc}.

%The intrinsic width of the $\PH_{5}$ boson is taken from the \texttt{H5plane} benchmark~\cite{LHCHiggsCrossSectionWorkingGroup:2016ypw} with the $s_{\mathrm{H}}$ values set to 0.5 for masses up to 0.8 TeV and 0.25 for higher massses. 



\begin{figure}[htbp]
\centering
\includegraphics[width=0.38\textwidth]{Figures/higgs_6TeV.pdf} 
\includegraphics[width=0.38\textwidth]{Figures/higgs_10TeV.pdf} 
\includegraphics[width=0.38\textwidth]{Figures/higgs_30TeV.pdf}
\caption{Distributions of $m_{\PV\PV}$ after the event selection for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV (upper left), 10 TeV (upper right), and 30 TeV (lower). The filled histograms show the background expectation, while the solid lines show the GM neutral Higgs signal predictions for values of $s_{\PH}=0.5$ and $m_{\PH_{5}}=500$ GeV (red), as well as for values $s_{\PH}=0.25$ and $m_{\PH_{5}}=1000$ GeV (green). Overflow is included in the last bin.\label{fig:dijet_mass_higgs}}
\end{figure}
%Distributions of $m_{\PW\PW}$ after the event selection in the $\PW\PW\nu\nu$ (left) and $\PW\PW\mu\mu$ (right) channels for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV (upper), $\sqrt{s}=10$ TeV (middle), and $\sqrt{s}=30$ TeV (lower). The filled histograms show the background expectation, while the solid lines show the separate contributions from the interference (red) and quadratic (green) terms for one illustrative aQGC parameter.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.45\textwidth]{Figures/heavy_higgs_xs_limit_6tev.png} 
\includegraphics[width=0.45\textwidth]{Figures/heavy_higgs_sh_limit_6tev.png}
\includegraphics[width=0.45\textwidth]{Figures/heavy_higgs_xs_limit_10tev.png} 
\includegraphics[width=0.45\textwidth]{Figures/heavy_higgs_sh_limit_10tev.png}
\includegraphics[width=0.45\textwidth]{Figures/heavy_higgs_xs_limit_30tev.png} 
\includegraphics[width=0.45\textwidth]{Figures/heavy_higgs_sh_limit_30tev.png}
\caption{Expected exclusion limits at 95\% CL for $\sigma (\PH_{5}\nu\nu) \mathcal{B}(\PH_{5} \to \PV\PV)$ (left) and for $s_{\PH}$ as a function of $m_{\PH_{5}}$ (right) in the GM model for a $\mu^{+}\mu^{-}$ collider with $\sqrt{s}=6$ TeV (upper), 10 TeV (middle), and 30 TeV (lower).\label{fig:gm_limits}}
\end{figure}



%The expected yields for the different SM processes and for an illustrative aQGC parameter in the $\PW\PW\nu\nu$ channel are given in Table~\ref{tab:yields_nunuWW}. The expected yield of the SM $\PW\PW\mu\mu$ contribution in the $\PW\PW\mu\mu$ channel is 10,703 while the expected yield of an illustrative aQGC parameter $f_{\text{T,1}}/ \Lambda^{4} = 1~\text{TeV}^{-4}$ is 265,307. 
%\begin{table}[htb]
%\centering
%\caption{The expected yields for various SM background processes in the $\PW\PW\nu\nu$ channel. The uncertainties due to the limited number of MC simulated events are negligible. \label{tab:yields_nunuWW}}

%\vspace{0.3cm}
%\begin{tabular}{lc}
%\toprule
%Process & Yields in $\PW\PW\nu\nu$ channel \\
%\midrule
%$\PW\PW\nu\nu$ & 1,082,800 \\
%\PW\PW\mu\mu$ & 11,181,200 \\
%$\PW\PZ\mu\nu$  & 1,132,800 \\
%$\PZ\PZ\mu\mu$ & 3,319 \\
%$\PW\PW\PZ$~$(\PZ\to\nu\nu)$ & 14,396 \\
%\midrule
%Total background & 12,331,715 \\
%$f_{\text{T,1}}/ \Lambda^{4} = 1~\text{TeV}^{-4}$ & 20,337,080 \\
%\bottomrule
%\end{tabular}
%\end{table}



% \begin{table}[htb]
% \centering
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators S0, S1, M0, M1, M7, T0, T1, and T2 in the $\PW\PW\nu\nu$ channel. \label{tab:limits_nunu}}
% \vspace{0.3cm}
% \begin{tabular}{cc}
% \toprule
% $\PW\PW\nu\nu$ & Limits (TeV\(^{-4}\)) \\
% \midrule
%  \(f_{\mathrm{M},0}/\Lambda^4\) & \([-0.032, 0.035]\) \\
%  \(f_{\mathrm{M},1}/\Lambda^4\) &  \([-0.088, 0.065]\)  \\
%  \(f_{\mathrm{M},7}/\Lambda^4\) &  \([-0.12, 0.17]\)  \\
%  \(f_{\mathrm{S},0}/\Lambda^4\) &  \([-0.22, 0.20]\) \\
%  \(f_{\mathrm{S},1}/\Lambda^4\) &  \([-0.14, 0.14]\) \\
%  \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.0062, 0.0030]\) \\
%  \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.0082, 0.0031]\) \\
%  \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.0096, 0.0046]\) \\
% \bottomrule
% \end{tabular}
% \end{table}




% \begin{table}[htb]
% \centering
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators T0, T1, T2, T6, T7 in the $\PW\PW\mu\mu$ channel at 6 TeV. \label{tab:limits_mumu}}
% \vspace{0.3cm}
% \begin{tabular}{ccc}
% \toprule
% $\PW\PW\nu\nu$ & Limits (TeV\(^{-4}\)) & Unitarity bound (TeV) \\
% \midrule
% \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.0065, 0.0026]\) & \([8.7, 10.9]\) \\
% \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.036, 0.024]\) & \([4.2, 5.2]\) \\
% \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.052, 0.030]\) & \([5.2, 6.7]\) \\
% \(f_{\mathrm{T},6}/\Lambda^4\) &  \([-0.0052, 0.0041]\) & \([10.0, 11.1]\) \\
% \(f_{\mathrm{T},7}/\Lambda^4\) &  \([-0.0068, 0.0042]\) & \([12.8, 15.0]\) \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators S0, S1, S2, M0, M1, M7, T0, T1, and T2 in the $\PW\PW\nu\nu$ channel at 10 TeV. \label{tab:limits_nunu}}
% \vspace{0.3cm}
% \begin{tabular}{ccc}
% \toprule
% $\PW\PW\nu\nu$ & Limits (TeV\(^{-4}\)) & Unitarity bound (TeV) \\
% \midrule
%  \(f_{\mathrm{M},0}/\Lambda^4\) & \([-0.0048, 0.0049]\) & \([8.9, 8.8]\)  \\
%  \(f_{\mathrm{M},1}/\Lambda^4\) &  \([-0.0096, 0.0084]\) & \([10.5, 10.8]\) \\
%  \(f_{\mathrm{M},7}/\Lambda^4\) &  \([-0.016, 0.019]\) & \([10.9, 10.6]\) \\
%  \(f_{\mathrm{S},0}/\Lambda^4\) &  \([-0.034, 0.033]\) & \([5.8, 6.8]\) \\
%  \(f_{\mathrm{S},1}/\Lambda^4\) &  \([-0.019, 0.019]\) & \([6.8, 6.6]\) \\
%  \(f_{\mathrm{S},2}/\Lambda^4\) &  \([-0.019, 0.019]\) & \([6.8,  6.6]\) \\
%  \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.00070, 0.00051]\) & \([10.0, 9.3]\) \\
%  \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.00089, 0.00053]\) & \([9.0, 10.3]\) \\
%  \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.0015, 0.0082]\) & \([10.8, 10.7]\) \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators T0, T1, T2, T6, T7 in the $\PW\PW\mu\mu$ channel at 10 TeV. \label{tab:limits_mumu}}
% \vspace{0.3cm}
% \begin{tabular}{ccc}
% \toprule
% $\PW\PW\nu\nu$ & Limits (TeV\(^{-4}\)) & Unitarity bound (TeV) \\
% \midrule
% \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.0012, 0.00057]\) & \([13.2, 15.8]\) \\
% \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.0020, 0.00089]\) & \([8.6, 11.9]\) \\
% \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.0068, 0.0012]\) & \([8.6, 15.1]\) \\
% \(f_{\mathrm{T},6}/\Lambda^4\) &  \([-0.00090, 0.00074]\) & \([15.5, 16.9]\) \\
% \(f_{\mathrm{T},7}/\Lambda^4\) &  \([-0.0011, 0.00086]\) & \([19.9, 22.3]\) \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators S0, S1, S2, M0, M1, M7, T0, T1, and T2 in the $\PW\PW\nu\nu$ channel at 30 TeV. \label{tab:limits_nunu}}
% \vspace{0.3cm}
% \begin{tabular}{ccc}
% \toprule
% $\PW\PW\nu\nu$ & Limits (TeV\(^{-4}\)) & Unitarity bound (TeV) \\
% \midrule
%  \(f_{\mathrm{M},0}/\Lambda^4\) & \([-0.00046, 0.00046]\) & \([15.8, 15.8]\)  \\
%  \(f_{\mathrm{M},1}/\Lambda^4\) &  \([-0.0012, 0.0011]\) & \([17.6, 17.8]\) \\
%  \(f_{\mathrm{M},7}/\Lambda^4\) &  \([-0.0021, 0.0022]\) & \([18.1, 17.9]\) \\
%  \(f_{\mathrm{S},0}/\Lambda^4\) &  \([-0.0046, 0.0045]\) & \([9.5, 10.9]\) \\
%  \(f_{\mathrm{S},1}/\Lambda^4\) &  \([-0.0025, 0.0025]\) & \([11.3, 10.9]\) \\
%  \(f_{\mathrm{S},2}/\Lambda^4\) &  \([-0.0025, 0.0025]\) & \([11.3, 10.9]\) \\
%  \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.000072, 0.000062]\) & \([17.7, 15.7]\) \\
%  \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.000095, 0.000082]\) & \([15.5, 16.3]\) \\
%  \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.00017, 0.00013]\) & \([18.4, 16.7]\) \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators T0, T1, T2, T6, T7 in the $\PW\PW\mu\mu$ channel at 30 TeV. \label{tab:limits_mumu}}
% \vspace{0.3cm}
% \begin{tabular}{ccc}
% \toprule
% $\PW\PW\nu\nu$ & Limits (TeV\(^{-4}\)) & Unitarity bound (TeV) \\
% \midrule
% \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.000031, 0.000018]\) & \([32.2, 36.8]\) \\
% \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.000050, 0.000031]\) & \([21.1, 27.0]\) \\
% \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.000091, 0.000042]\) & \([24.8, 35.1]\) \\
% \(f_{\mathrm{T},6}/\Lambda^4\) &  \([-0.000027, 0.000024]\) & \([37.1, 40.1]\) \\
% \(f_{\mathrm{T},7}/\Lambda^4\) &  \([-0.000034, 0.000028]\) & \([47.8, 52.7]\) \\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}[htb]
% \caption{Expected lower and upper 95\% CL limits on the parameters of the quartic operators T0, T1, T2, T6, and T7 in the $\PW\PW\mu\mu$ channel.}
% \label{tab:limits_mumu}
% \vspace{0.3cm}
% \centering
% \begin{tabular}{c c}
% \toprule
% $\PW\PW\mu\mu$ &  Limits (TeV\(^{-4}\)) \\
% \hline
%  \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.04, 0.028]\) \\
%  \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.025, 0.0095]\)  \\
%  \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.12, 0.068]\)  \\
%  \(f_{\mathrm{T},6}/\Lambda^4\) &  \([-0.034, 0.033]\) \\
%  \(f_{\mathrm{T},7}/\Lambda^4\) &  \([-0.043, 0.038]\) \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htb]
% \caption{[UPDATED TABLE] Expected lower and upper 95\% CL limits on the parameters of the quartic operators T0, T1, T2, T6, and T7 in the $\PW\PW\mu\mu$ channel.}
% \label{tab:limits_mumu}
% \vspace{0.3cm}
% \centering
% \begin{tabular}{c c}
% \toprule
% $\PW\PW\mu\mu$ &  Limits (TeV\(^{-4}\)) \\
% \hline
%  \(f_{\mathrm{T},0}/\Lambda^4\) &  \([-0.02, 0.01]\) \\
%  \(f_{\mathrm{T},1}/\Lambda^4\) &  \([-0.03, 0.01]\)  \\
%  \(f_{\mathrm{T},2}/\Lambda^4\) &  \([-0.06, 0.02]\)  \\
%  \(f_{\mathrm{T},6}/\Lambda^4\) &  \([-0.01, 0.01]\) \\
%  \(f_{\mathrm{T},7}/\Lambda^4\) &  \([-0.02, 0.01]\) \\
% \bottomrule
% \end{tabular}
% \end{table}

%\begin{table}[htb]
%\caption{TODO: appropriate caption for neutral heavy higgs limits.}
%\label{tab:limits_heavyHiggs}
%\vspace{0.3cm}
%\centering
%\scriptsize
%\begin{tabular}{c c c c}
%\toprule
%Neutral heavy Higgs mass (GeV) &  sh Limits (6 TeV CM) &  sh Limits (10 TeV CM) & sh Limits (30 TeV CM)\\
%\hline
% 500 & 0.11 & 0.071 & 0.062 \\
% 600 & 0.075 & 0.048 & 0.042  \\
% 700 & 0.059 & 0.038 & 0.034  \\
% 800 & 0.043 & 0.029 & 0.026 \\
% 900 & 0.069 & 0.045 & 0.041 \\
% 1000 & 0.055 & 0.036 & 0.034 \\
% 2000 & 0.018 & 0.012 & 0.011 \\
% 3000 & 0.012 & 0.006 & 0.006 \\
%\bottomrule
%\end{tabular}
%\end{table}




%For the aQGC limits, we use the following profile likelihood test statistic: \[t_{\alpha}=2 \log\left(\frac{L(\alpha}{L(\hat{\alpha})}\right)\]
%Only statistical uncertainty is accounted for; no nuisance parameters corresponding to systematic uncertainties are included. \(\alpha\) corresponds to the aQGC strength being tested, while \(\hat{\alpha}\) corresponds to the aQGC strength for which the likelihood function is maximized. The test statistic is assumed to follow a noncentral \(\chi^2\) distribution, from which it follows that the 95\% confidence level (CL) limits on aQGC parameters are found for \(t_{\alpha}=-2\Delta\log(L)=3.84\) \cite{wilks:10.1214}. 

%To find the expected 95\% CL limits on each aQGC parameter, shown in Table \ref{tab:limits}, we vary each aQGC parameter separately, with all others set to the SM value of 0. Figure \ref{fig:nunu_M0_scan} shows such a scan performed for the \(M_0\) operator.




% - one likelihood scan plot for each channel 
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.8]{c_scan_M0.pdf}
%    \caption{Expected 95\% CL interval on the aQGC parameter \(f_{M_0} / \Lambda^4\)}
%    \label{fig:nunu_M0_scan}
%\end{figure}



==> Sections/selection.tex <==
\section{Event selection}
\label{S:sel}

Events are selected targeting hadronically-decaying $\PW\PW$ and $\PZ\PZ$ boson pairs with a large invariant mass. The jets are required to have transverse momenta ($\pt$) greater than 100 GeV and be relatively central, with $|\cos \theta| < 0.8$, where $\theta$ is the angle of the jet with respect to the beam axis. The jet with the highest $\pt$ is called the ``leading jet'' and the jet with the second-highest $\pt$ the ``subleading jet.'' The leading and subleading jets are each required to have a mass greater than 40 GeV.

%, to select collimated $V\rightarrow qq^{\prime}$ decays contained within a single jet.

The $\PW\PW\nu\nu$ and $\PZ\PZ\nu\nu$ channels are targeted by vetoing events with a reconstructed electron or muon with momentum greater than $3$ GeV. This requirement significantly reduces the $\PW\PW\mu\mu$ and $\PZ\PZ\mu\mu$ background contributions in these channels, which could be reduced even further with a detector with better forward muon coverage. As these channels contain two neutrinos in the final state, the events are also required to have a missing mass ($m_\mathrm{miss}$) greater than $200$ GeV. The $m_\mathrm{miss}$ is defined as   
\begin{equation}
m_\mathrm{miss} = \sqrt{(\sqrt{s}-E_{\PV\PV})^2-|\vec{p}_{\PV\PV}|^{2}},
\label{eq:missingmass}
\end{equation}
where $E_{\PV\PV}$ and $\vec{p}_{\PV\PV}$ are the energy and momentum of the $\PV$ boson pair. This requirement removes events where neutrinos are produced from $\PZ$ boson decays and reduces the contributions of the s-channel $\PW\PW$ and two-jet processes.

The $\PW\PW\mu\mu$ channel is targeted by requiring two oppositely-charged muons with momenta greater than $0.5$ GeV and $|\cos \theta| < 0.99$. The largely dominant background contribution is the SM production of $\PW\PW\mu\mu$ where the final state muons tend to be very forward. The mass of the dimuon pair is required to be greater than 106 GeV to reduce the contribution of events where the muons are produced from $\PZ$ boson decays.
